Robust Cross-Modal Representation Learning with Progressive Self-Distillation

The learning objective of vision-language approach of CLIP does not effectively account for the noisy many-to-many correspondences found in web-harvested image captioning datasets, which contributes to its compute and data inefficiency. To address this challenge, we introduce a novel training framework based on cross-modal contrastive learning that uses progressive self-distillation and soft image-text alignments to more efficiently learn robust representations from noisy data. Our model distills its own knowledge to dynamically generate soft-alignment targets for a subset of images and captions in every minibatch, which are then used to update its parameters. Extensive evaluation across 14 benchmark datasets shows that our method consistently outperforms its CLIP counterpart in multiple settings, including: (a) zero-shot classification, (b) linear probe transfer, and (c) image-text retrieval, without incurring added computational cost. Analysis using an ImageNet-based robustness test-bed reveals that our method offers better effective robustness to natural distribution shifts compared to both ImageNet-trained models and CLIP itself. Lastly, pretraining with datasets spanning two orders of magnitude in size shows that our improvements over CLIP tend to scale with number of training examples.

==> figures/figure_robustness_examples.tex <==
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/robustness_supp.pdf}
    \caption{
    \small
    \textbf{Robustness Examples --} Given an image from the ImageNet-R dataset (left column), we compare the predictions of CLIP (middle column) to the predictions of our method (right column) by showing the probabilities assigned to the top 5 classes.
    }
    \label{fig:robustness}
\end{figure*}

==> figures/figure_sim_visualization.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/similarity_vis.png}
    \caption{
    Visualization of our method's similarity scores between a batch of four image-text pairs. The baseline CLIP is optimized to maximize the diagonal scores and minimize off-diagonal scores. Our method yields elevated similarity scores on off-diagonal elements when there is increased semantic similarity between unpaired instances (e.g., photographer-to-astronaut pairing and the black-and-white-to-photographer-to-page of text pairing).
    }
    \label{fig:similarity_vis}
\end{figure}

==> tables/eval_datasets.tex <==
\begin{table}[h!]
    \centering
    \begin{tabular}{lccc}
    \hline
    \textbf{Dataset} & \textbf{Classes} & \textbf{Train Size} & \textbf{Test Size} \\
    \hline
    Cifar10    & 10   & 50,000    & 10,000 \\
    Cifar100   & 100  & 50,000    & 10,000 \\
    Caltech101 & 102  & 2,863     & 8,677 \\
    Food101    & 101  & 75,750    & 25,250 \\
    OxfordPets & 37   & 3,680     & 3,669  \\
    Birdsnap   & 500  & 38,344    & 1,900  \\
    ImageNet   & 1000 & 1,281,167 & 50,000 \\
    Places365  & 365  & 1,803,460 & 36,489 \\
    ObjectNet  & 313  & -         & 50,000 \\
    ImageNet-A & 200  & -         & 7,500  \\
    ImageNet-O & 200  & -         & 2,000  \\
    ImageNet-R & 200  & -         & 30,000 \\
    ImageNetV2 & 1000 & -         & 30,000 \\
    
    \hline
    \end{tabular}
    \caption{\textbf{Evaluation Dataset Details --} The number of classes, training and testing examples present in the evaluation datasets. The size of the training set size for the last 5 rows is omitted because these datasets are designated as ``testing-only'' benchmarks.}
    \label{tab:eval_datasets}
\end{table}



==> tables/hparams.tex <==

\begin{table}[h!]
    \centering
    \begin{tabular}{lc}
    \toprule
    \textbf{Hyperparameter}            & \textbf{Value}     \\
    \midrule
    Batch size                         & 4096               \\
    Vocabulary size                    & 49408              \\
    Training epochs                    & 100                \\
    Initial temperature $\tau$         & 0.07               \\
    Teacher temperature $\tilde{\tau}$ & 0.1                \\
    Weight decay                       & 0.001              \\
    Warm-up iterations (\%)            & 0.2                \\
    Learning rate                      & $1 \times 10^{-5}$ \\
    Adam $\beta_1$                     & 0.9                \\
    Adam $\beta_2$                     & 0.99               \\
    Adam $\epsilon$                    & $10^{-5}$          \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Common hyperparameters --} used for both baseline CLIP pretraining and our method.}
    \label{tab:hparams}
	
\end{table}


==> tables/pretraining_datasets.tex <==
\begin{table}[h!]
    \centering
    \begin{tabular}{c|ccc}
    \hline
    \textbf{Dataset} & \textbf{COCO} & \textbf{CC3M} & \textbf{CC12M} \\
    \hline
    \# & 118,287  & 2,884,940  & 10,707,814 \\
    \hline
    \end{tabular}
    \caption{\textbf{Pretraining Dataset Sizes --} Exact sizes of pretraining datasets employed in this work (no. of image-text pairs). }
    \label{tab:pretraining_datasets}
\end{table}



==> tables/prompts.tex <==

\begin{table*}[h!]
    \centering
    \begin{tabular}[t!]{l|l|l}
    \hline
    \small
    \textbf{Cifar\{10,100\}} &
    \textbf{Caltech101} &
    \textbf{ImageNet+}              \\
    \hline
    \scriptsize{\shortstack[l]{
    ''a photo of a \{\}.'',\\
    ''a blurry photo of a \{\}.'',\\
    ''a black and white photo of a \{\}.'',\\
    ''a low contrast photo of a \{\}.'',\\
    ''a high contrast photo of a \{\}.'',
    ''a bad photo of a \{\}.'',\\
    ''a good photo of a \{\}.'',
    ''a photo of a small \{\}.'',\\
    ''a photo of a big \{\}.'',
    ''a photo of the \{\}.'',\\
    ''a blurry photo of the \{\}.'',
    ''a black and white photo of the \{\}.'',\\
    ''a low contrast photo of the \{\}.'',
    ''a high contrast photo of the \{\}.'',\\
    ''a bad photo of the \{\}.'',
    ''a good photo of the \{\}.'',\\
    ''a photo of the small \{\}.'',
    ''a photo of the big \{\}.''
    }}
    &
    \scriptsize{
    \shortstack[l]{
    ``a photo of a \{\}.'',
    ``a painting of a \{\}.'',
    ``a plastic \{\}.'',\\
    ``a sculpture of a \{\}.'',
    ``a sketch of a \{\}.'', 
    ``a tattoo of a \{\}.'',\\
    ``a toy \{\}.'',
    ``a rendition of a \{\}.'',
    ``a embroidered \{\}.'',
    ``a cartoon \{\}.'',\\
    ``a \{\} in a video game.'',
    ``a plushie \{\}.'',
    ``a origami \{\}.'',
    ``art of a \{\}.'',\\
    ``graffiti of a \{\}.'',
    ``a drawing of a \{\}.'',
    ``a doodle of a \{\}.'',\\
    ``a photo of the \{\}.'',
    ``a painting of the \{\}.'',
    ``the plastic \{\}.'',\\
    ``a sculpture of the \{\}.'',
    ``a sketch of the \{\}.'',
    ``a tattoo of the \{\}.'',\\
    ``the toy \{\}.'',
    ``a rendition of the \{\}.'',
    ``the embroidered \{\}.'',\\
    ``the cartoon \{\}.'',
    ``the \{\} in a video game.'',
    ``the plushie \{\}.'',\\
    ``the origami \{\}.'',
    ``art of the \{\}.'',
    ``graffiti of the \{\}.'',\\
    ``a drawing of the \{\}.'',
    ``a doodle of the \{\}.''
    }}
    &
    \footnotesize{
    \shortstack[l]{
    ``\{\}''\\
    ``A photo of \{\}''\\
    ``A photo the \{\}''\\
    ``itap of a \{\}.''\\
    ``a bad photo of the \{\}.''\\
    ``a origami \{\}.''\\
    ``a photo of the large \{\}.''\\
    ``a \{\} in a video game.''\\
    ``art of the \{\}.''\\
    ``a photo of the small \{\}.''
	}} \\
    \hline
    \end{tabular}
    \caption{\textbf{Prompt templates for zero-shot evaluation --} The placeholder symbol \{\} is replaced with a string representation of the category name. The last column ``ImageNet+'' corresponds to the templates used for all other datasets that appear in this work, including all of the ImageNet variants. }
    \label{tab:prompts}
	
\end{table*}


==> tables/results_rn50.tex <==


\begin{table*}[!h]
    \vspace{-5mm}
	\small{
    \centering
    \begin{tabular}{ccccccccccccl}
    \small{\shortstack[c]{Pretraining\\ Dataset}} &
    \small{\shortstack[c]{Method}} &
    \rotatebox{70}{\tiny{Cifar10}} &
    \rotatebox{70}{\tiny{Cifar100}} &
    \rotatebox{70}{\tiny{Caltech101}} &
    \rotatebox{70}{\tiny{Places365}} &
    \rotatebox{70}{\tiny{ObjectNet}} &
    \rotatebox{70}{\tiny{ImageNet-R}} &
    \rotatebox{70}{\tiny{ImageNet-O}} &
    \rotatebox{70}{\tiny{Imagenet-A}} &
    \rotatebox{70}{\tiny{ImageNetV2}} &
    \rotatebox{70}{\tiny{ImageNet}} &
    \rotatebox{70}{\tiny{Average}} \\
    \midrule
    \multirow{2}{*}{COCO}     & CLIP & 31.12 & 7.66 & 27.01 & 10.56 & 2.64 & 5.77  & 8.9  & 2.31 & 5.92 & 6.59 & 10.84 \\
                              & Ours & \textbf{37.85} & \textbf{9.97} & \textbf{33.87} & \textbf{11.17} & \textbf{3.38}& \textbf{6.48} & \textbf{11.7}& \textbf{2.56}& \textbf{6.87}& \textbf{7.48}& $\textbf{13.12}^{\textbf{\textcolor{mygreen}{+2.27}}}$ \\
    \cdashline{1-13}
    \multirow{2}{*}{CC3M}     & CLIP & 36.46 & 14.20 & 44.81 & 19.29 & 3.24 & 19.28 & 24.50 & 3.53 & 16.95 & 18.12  & 20.04 \\
                              & Ours & \textbf{56.69} & \textbf{24.44} & \textbf{61.93} & \textbf{24.67} & \textbf{5.27} &\textbf{25.96} & \textbf{31.65} & \textbf{4.57} & \textbf{21.65} & \textbf{22.918} & $\textbf{27.98}^{\textbf{\textcolor{mygreen}{+7.94}}}$ \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Zero-Shot Image Classification Comparison with RN50 backbone -- } Zero-shot Top1 accuracy (\%) of our method compared to baseline CLIP on numerous downstream benchmark datasets. Note: Results are derived from published hyperparameters for the baseline and minimal hyperparameter tuning of our method to account for differences in backbone architecture.}
    \label{tab:results}
	}
\end{table*}



==> tables/table_comparison.tex <==
\begin{table}[H]
	\small{
    \centering
    \begin{tabular}{lllc}
    \toprule
    \shortstack[c]{\textbf{Dataset}} &
    \shortstack[c]{\textbf{Method}} &
   \textbf{Architecture} &
   \textbf{ImageNet} \\
    \midrule
    \multirow{10}{*}{YFCC (15M)}     & CLIP impl.~\cite{yao2021filip}               & ViT-B/32 & 30.4 \\
                                     & FILIP~\cite{yao2021filip}                    & ViT-B/32 & 37.8 \\
                                     & CLOOB~\cite{furst2021cloob}                  & RN50     & 35.7 \\
                                     & CLOOB~\cite{furst2021cloob}                  & RN101    & 37.1 \\
                                     & CLOOB~\cite{furst2021cloob}                  & RN50x4   & 39.0 \\
                                     & CLIP impl.~\cite{li2021supervision}          & RN50     & 35.9 \\
                                     & DeCLIP~\cite{li2021supervision}              & RN50     & 41.9 \\
                                     & OpenAI CLIP~\cite{radford2021learning}       & RN50     & 31.3 \\
                                     & OpenCLIP~\cite{ilharco_gabriel_2021_5143773} & RN50     & 32.7 \\
                                     & OpenCLIP~\cite{ilharco_gabriel_2021_5143773} & RN101    & 34.8 \\
    \cdashline{1-4}
    \multirow{7}{*}{CC3M}     & OpenCLIP~\cite{ilharco_gabriel_2021_5143773} & RN50x4   & 22.2 \\
                              & CLIP impl.~\cite{furst2021cloob}             & RN50     & 23.9 \\ 
                              & CLOOB~\cite{furst2021cloob}                  & RN50     & 25.6 \\
                              & DeCLIP~\cite{li2021supervision}              & RN50     & 27.8 \\
                              & CLIP impl. (ours)                            & ViT-B/32 & 23.5 \\
                              & \textbf{Our method}                          & ViT-B/32 & \textbf{28.0} \\
    \cdashline{1-4}
    \multirow{3}{*}{CC12M}     & CLIP impl. (ours)               & ViT-B/32 & 37.8          \\
                               & DeCLIP~\cite{li2021supervision} & RN50     & 41.0          \\ 
                               & \textbf{Our method}             & ViT-B/32 & \textbf{42.2} \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Zero-Shot ImageNet Classification Comparison -- } Zero-shot Top1 accuracy (\%) of our method compared to concurrent works.}
    \label{tab:zeroshot_comparison}
	}
\end{table}


